Dispelling Myths on Superposition Attacks: Formal Security Model and Attack Analyses

It is of folkloric belief that the security of classical cryptographic protocols is automatically broken if the Adversary is allowed to perform superposition queries and the honest players forced to perform actions coherently on quantum states. Another widely held intuition is that enforcing measurements on the exchanged messages is enough to protect protocols from these attacks. However, the reality is much more complex. Security models dealing with superposition attacks only consider unconditional security. Conversely, security models considering computational security assume that all supposedly classical messages are measured, which forbids by construction the analysis of superposition attacks. Boneh and Zhandry have started to study the quantum computational security for classical primitives in their seminal work at Crypto'13, but only in the single-party setting. To the best of our knowledge, an equivalent model in the multiparty setting is still missing. In this work, we propose the first computational security model considering superposition attacks for multiparty protocols. We show that our new security model is satisfiable by proving the security of the well-known One-Time-Pad protocol and give an attack on a variant of the equally reputable Yao Protocol for Secure Two-Party Computations. The post-mortem of this attack reveals the precise points of failure, yielding highly counter-intuitive results: Adding extra classical communication, which is harmless for classical security, can make the protocol become subject to superposition attacks. We use this newly imparted knowledge to construct the first concrete protocol for Secure Two-Party Computation that is resistant to superposition attacks. Our results show that there is no straightforward answer to provide for either the vulnerabilities of classical protocols to superposition attacks or the adapted countermeasures.

==> tex_files/A2_IF.tex <==
We present here the 1-out-of-2 String Oblivious 
Transfer Ideal Functionality (Ideal Functionality \ref{IdealOT}), in which one 
party ($\Pone$ in our case) has two strings $(k_0, k_1)$ and the other 
($\Ptwo$) has a bit $b \in \{0, 1\}$. The output of $\Ptwo$ is the string 
$k_b$ (with no knowledge about $k_{\bar{b}}$), while on the other hand $\Pone$ 
has no output and no knowledge about choice-bit $b$.

\begin{idealf}
\caption{1-out-of-2 String OT.}
\label{IdealOT}
\begin{itemize}

\item \textbf{Inputs:} $\Pone$ has as input $(k_0, k_1)$ and $\Ptwo$ has as input $b \in \{0, 1\}$.

\item \textbf{Computation by the trusted party:}
\begin{enumerate} 
\item If the trusted party receives $\Abort$ or an incorrectly formatted input from either party, it sends $\Abort$ to both parties and halts.
\item Otherwise, let $(\widehat{k_0}, \widehat{k_1})$ and $\hat{b}$ be the inputs received. The Ideal Functionality sends $\widehat{k_{\hat{b}}}$ to $\Ptwo$ and halts.
\end{enumerate} 
\end{itemize}
\end{idealf}
